A velocity-entropy invariance theorem for the Chapman-Jouguet detonation

The velocity and specific entropy of the Chapman-Jouguet (CJ) equilibrium detonation are shown to be invariant under the same variations of initial temperature with initial pressure. This leads to additional CJ relations, for example, for calculating the CJ state -- including the adiabatic exponent -- from the only CJ velocity, without using an equation of state for the detonation products. For gaseous stoichiometric explosives with ideal products, numerical calculations with detailed chemical equilibrium confirm the invariance theorem to $\mathcal{O}(10^{-2}$\% and the additional CJ properties to $\mathcal{O}(10^{-1}$\%. However, for four liquid carbon explosives, the predicted CJ pressures are about 20\% higher than the measurements. The analysis emphasizes the limited physical representativeness of the hydrodynamic framework of the modelling, i.e. single-phase inviscid fluids at equilibrium for the initial and final states of the explosive. This invariance may illustrate a general feature of hyperbolic systems and their characteristic surfaces.

==> Acknowledgments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{\label{sec:Acknow}Acknowledgments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This work is dedicated to the memory of Dr. Michael Cowperthwaite.

==> VIII_C_A_model_problem.tex <==
%newline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\label{sec:ModPb}A model problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let the differentials of the functions $\beta \left(
w,x\right) $ and $\sigma \left( w,x\right) $ of the two variables $w$ and $x$
satisfy%
\begin{align}
\varepsilon d\beta &=adw+bdx,  \label{C1} \\
d\sigma &=qdw+rdx,  \label{C2}
\end{align}%
where $\varepsilon $, $a$, $b$, $q$, $r$ are finite functions of $\beta $, $%
w $ and $x$. These relations define the constraints%
\begin{align}
\varepsilon \left. \frac{\partial \beta }{\partial x}\right) _{w} &=b,
\label{C3} \\
\varepsilon \left. \frac{\partial \beta }{\partial x}\right) _{\sigma }
&=a\left. \frac{\partial w}{\partial x}\right) _{\sigma }+b,  \label{C4} \\
0 &=q\left. \frac{\partial w}{\partial x}\right) _{\sigma }+r.  \label{C5}
\end{align}%
The last, (\ref{C5}), is the triple product rule, given that (\ref%
{C2}) is a total differential, that is,
\begin{align}
&d\sigma =\left. \frac{\partial \sigma }{\partial w}\right) _{x}dw+\left. 
\frac{\partial \sigma }{\partial x}\right) _{w}dx  \label{TWO_VAR_ID_APP_1}
\\
&\Rightarrow \left. \frac{\partial \sigma }{\partial x}\right) _{w}=-\left. 
\frac{\partial \sigma }{\partial w}\right) _{x}\left. \frac{\partial w}{%
\partial x}\right)_{\sigma }\Leftrightarrow r=-q\left. \frac{\partial w}{\partial x}\right) _{\sigma }.
\label{TWO_VAR_ID_APP_3}
\end{align}%
Therefore, if either $\left. \partial w/\partial x\right) _{\sigma }$ or $%
\left. \partial \sigma /\partial x\right) _{w}\equiv r$ is zero, so is the
other if $\left. \partial \sigma /\partial w\right) _{x}\equiv q$ is finite
and non-zero.

In the limit $\varepsilon=0$, (\ref{C3}) shows that $b^{(\varepsilon=0)}=0$
if $\left. \partial \beta /\partial x\right) _{w}^{(\varepsilon=0)}$ is
finite, then (\ref{C4}) shows that $\left. \partial w /\partial x\right) _{\sigma}^{(\varepsilon=0)}=0$ if $\left. \partial \beta /\partial x\right) _{\sigma }^{(\varepsilon=0)}$ is
finite and\ $a^{(\varepsilon=0)}$ is finite and $\neq 0$, then (\ref{C5})
shows that%
\begin{equation}
\text{ }\left. \frac{\partial \sigma }{\partial x}\right) _{w}^{(\varepsilon=0
)}\equiv r^{(\varepsilon=0 )}=0\Leftrightarrow \left. \frac{\partial w}{%
\partial x}\right) _{\sigma }^{\left(\varepsilon=0\right) }\hspace{-0.15cm}=0
\end{equation}%
if $q^{(\varepsilon=0 )}\equiv \left. \partial \sigma /\partial w\right)
_{x}^{\left(\varepsilon=0 \right) }\hspace{-0.15cm}$ \ is finite and $\neq 0$, hence, with (\ref{TWO_VAR_ID_APP_1}), the equivalence $\left( d\sigma \right) ^{(\varepsilon=0)}=0\Leftrightarrow
\left( dw\right) ^{(\varepsilon=0)}=0$.
%, but not that $\left( d\sigma \right) ^{(\varepsilon=0)}$ or $\left( dw\right) ^{(\varepsilon=0)}$ is zero. %
The theorem \hyperref[subsec:Proof]{(Subsect. III-C)} is the application for which $\varepsilon =1-M$, $%
\sigma =s$, $\beta =v$, $p$ or $h$, $w=D$, $x=v_{0}$, $a\propto K_{z}\neq 0$%
, $q\propto K_{s}\neq 0$, $b\propto \Phi _{z}^{\ast }$ and $r\propto \Phi
_{s}^{\ast }$.\newline

If the arguments of $b\left( \beta ,w,x\right) $ and $r\left( \beta ,w,x\right) $ include the same grouping $\mu _{0}\left( \beta,w,x\right) $, and, in conditions for which $\left( d\sigma \right)
^{(\varepsilon=0)}=0$ or $\left( dw\right) ^{(\varepsilon=0)}=0$, eliminating $%
\mu _{0}$ between the constraint $%
b^{(\varepsilon=0)}\left( \beta ,w,x,\mu _{0}\right) =0$ and $r^{(\varepsilon=0
)}\left( \beta ,w,x,\mu _{0}\right) =0$ defines the compatibility relation $\beta =\beta ^{\left(
\varepsilon=0\right) }\left( w,x\right) $, which substituted for $\beta $ in either of these constraints then returns $\mu_{0}^{\left( \varepsilon=0\right) }$. These are the operations in \hyperref[subsec:CJsuppl]{subsection  III-D} that give $v_{\text{CJ}}/v_{0}$ and $dp_{0}^{\ast }/dv_{0}$, here represented by $\mu_{0}$.
\newline\newline

% The \nocite command causes all entries in a bibliography to be printed out
% whether or not they are actually referenced in the text. This is appropriate
% for the sample file to show the different styles of references, but authors
% most likely will not want to use it.
%\nocite{*}
